Unclonable Secret Sharing

Unclonable cryptography utilizes the principles of quantum mechanics to addresses cryptographic tasks that are impossible classically. We introduce a novel unclonable primitive in the context of secret sharing, called unclonable secret sharing (USS). In a USS scheme, there are $n$ shareholders, each holding a share of a classical secret represented as a quantum state. They can recover the secret once all parties (or at least $t$ parties) come together with their shares. Importantly, it should be infeasible to copy their own shares and send the copies to two non-communicating parties, enabling both of them to recover the secret. Our work initiates a formal investigation into the realm of unclonable secret sharing, shedding light on its implications, constructions, and inherent limitations. ** Connections: We explore the connections between USS and other quantum cryptographic primitives such as unclonable encryption and position verification, showing the difficulties to achieve USS in different scenarios. **Limited Entanglement: In the case where the adversarial shareholders do not share any entanglement or limited entanglement, we demonstrate information-theoretic constructions for USS. **Large Entanglement: If we allow the adversarial shareholders to have unbounded entanglement resources (and unbounded computation), we prove that unclonable secret sharing is impossible. On the other hand, in the quantum random oracle model where the adversary can only make a bounded polynomial number of queries, we show a construction secure even with unbounded entanglement. Furthermore, even when these adversaries possess only a polynomial amount of entanglement resources, we establish that any unclonable secret sharing scheme with a reconstruction function implementable using Cliffords and logarithmically many T-gates is also unattainable.

==> append_IT_imposibility_full.tex <==
\section{Full Attack Description for the Impossibility Result in Information-theoretic Setting}
\label{sec:app_it_impossibility_full}

\jiahui{put in an algorithm box?}

\begin{proof}[Proof]
%Based on port-based teleportation.
We number the parties to be $P_1, \cdots, P_n$. They are all unbounded in computational resources, storage and communication size.


Suppose there exists an information-theoretically secure USS scheme for ${\cal P}$. In order to recover the secret, one needs to apply a POVM $\{\reconstruct^\gamma_{P_1\cdots P_n}\}_{\gamma}$ to $\rho_1, \cdots, \rho_n$ and output (w.l.o.g.) the first $|m|$-bit as secret $\hat{m} \in \{0,1\}^{|m|}$ in the measurement outcome.
\par We construct an adversary ${\cal P}$ that take as input a shared joint state $\ket{\Psi}_{\sfP_1,\cdots \sfP_n} \in \bigotimes_i^{n} (\mathbb{C}^2)^{\otimes k}$. We denote $\rho_1,\cdots,\rho_n$ to be the reduced density matrices of all the adversarial parties.
\jiahui{revised}

 %Suppose that the protocol gives shares an $k$-qubit state $\rho_1, \cdots, \rho_n$ to parties $P_1, \cdots, P_n$ respectively. We view the entire system of all parties as a state $\ket{\Psi}_{P_1,P_2\cdots P_n} \in \bigotimes_i^{n} (\mathbb{C}^2)^{\otimes k}$ (as a pure state for the purpose of cleaner notations, since our attack works regardless of this joint state being mixed or pure).
%In order to recover the secret, one needs to apply a POVM $\{\reconstruct^\gamma_{P_1\cdots P_n}\}_{\gamma}$ to $\rho_1, \cdots, \rho_n$ and output (w.l.o.g.) the first $|m|$-bit as secret $\hat{m} \in \{0,1\}^{|m|}$ in the measurement outcome. \pnote{some notational inconsistencies need to be fixed: for registers, use bold or calligraphic letters everywhere. Use $\adv$ instead of $P_1,\ldots,P_n$ to denote an adversary.}

\noindent \pnote{how about rephrasing the above as follows? 
Suppose there exists an information-theoretically secure USS scheme for ${\cal P}$. In order to recover the secret, one needs to apply a POVM $\{\reconstruct^\gamma_{P_1\cdots P_n}\}_{\gamma}$ to $\rho_1, \cdots, \rho_n$ and output (w.l.o.g.) the first $|m|$-bit as secret $\hat{m} \in \{0,1\}^{|m|}$ in the measurement outcome.
\par We construct an adversary ${\cal P}$ that take as input a shared joint state $\ket{\Psi}_{P_1,\cdots P_n} \in \bigotimes_i^{n} (\mathbb{C}^2)^{\otimes k}$. We denote $\rho_1,\cdots,\rho_n$ to be the reduced density matrices of all the adversarial parties. 



%Suppose that the protocol gives shares an $k$-qubit state $\rho_1, \cdots, \rho_n$ to parties $P_1, \cdots, P_n$ respectively. We view the entire system of all parties as a state $\ket{\Psi}_{P_1,P_2\cdots P_n} \in \bigotimes_i^{n} (\mathbb{C}^2)^{\otimes k}$ (as a pure state for the purpose of cleaner notations, since our attack works regardless of this joint state being mixed or pure).
% \pnote{not sure I follow this sentence: I think it can be removed since it doesn't affect the formal description below.}
}

With a slight abuse of notations, we name the register that holds the state $\rho_i$ as $\sfP_i$.


%for each $i \in [n]$, \pnote{incomplete sentence}\\

\noindent The attack strategy is as follows:
\jiahui{My plan now is: first write a less formal proof with simple notations as an overview (apart from technical overview and then followed by this "actual attack"}
\pnote{I had trouble following the text below due to the usage of many registers: is it necessary for us to state how many registers each party has and so on? can't we just say that the parties share xyz EPR pairs and after performing port-teleportation, they have abc state with the following form etc.? if we can avoid using notation for registers, we should. If it helps to discuss before polishing, let me know.\\

\noindent Also, it is assumed that $P_1$ is "connected" with everyone else: I couldn't find this explicitly mentioned anywhere. }
\jiahui{mentioned in the following setup.}

%\paragraph{Notation} 

\begin{enumerate}
    \item Setup:

    \begin{enumerate}
        \item  For each $i \in [n], i \neq 1$, $P_i$ shares $k$ qubits of entanglement with $P_1$ in registers $\sfP_i': \sfP_{1,i}'$ \footnote{We denote registers $\mathsf{X}: \mathsf{Y}$ as a pair of registers which hold a pair of maximally entangled states.};
        %\pnote{what does $X:Y$ mean?}\pnote{define an ebit}
        

        \item Additionally, for each "neighboring" two parties $i$ and  $i+1$, they hold additional $N_{i,i+1}$ registers: $\sfP_{i,R,\ell_{i,i+1}}:\sfP_{i+1,L, \ell_{i,i+1}}$, each with $nk$ qubits of maximal entanglement, for all $\ell_{i,i+1} \in [N_{i,i+1}]$ (We will specify the quantity for $N_{i,i+1}$ later).
        We denote $\sfP_{i, R}^{N_{i,i+1}} := \sfP_{i,R,1} \sfP_{i,R,2} \cdots \sfP_{i,R,N_{i,i+1}}$ and $\sfP_{i+1,L}^{N_{i,i+1}} := \sfP_{i+1,L,1} \sfP_{i+1,L,2} \cdots \sfP_{i+1,L,N_{i,i+1}}$.
    \end{enumerate}

    \item Regular teleportation stage:
    
    \begin{enumerate}
        \item   For each party $P_i, i \in [n], i \neq 1$, $P_i$ performs a regular teleportation measurement on registers $\sfP_i:\sfP_i'$ to obtain measurement outcome $\sigma_i$. We also accordingly denote the Pauli operators that will appear upon the teleported state in $P_1$'s side as $\sigma_i$.  
    
    \item As a result, now party $P_1$ holds an $n$-partite state $(\mathbb{I} \otimes \sigma_2 \otimes\cdots \otimes \sigma_n) \ket{\Psi}_{\sfP_1, \sfP_{1,2}',\cdots \sfP_{1,n}'}$ in registers $\sfP_1,\sfP_{1,2}',\cdots \sfP_{1,n}'$.
    \end{enumerate}


    \item Port-based teleportation stage:
    
    For clarity, we first describe the part of the protocol performed by party $P_1$ and party $P_2$. Then we generlize to the rest of the parties.
    \begin{enumerate}
        \item     $P_1$ now performs a port-based teleportation measurement on its $nk$-qubits in registers $\sfP_1, \sfP_{1,2}',\cdots \sfP_{1,n}'$ and its part of the shared entanglement $\sfP_{1}^{N_{1,2}}: \sfP_{2}^{N_{1,2}}$.
    Party $P_1$ obtains a measurement outcome $\ell_{1,2}^*$, which is an index in $[1,2,\cdots, N_{1,2}]$. 
    Now, party $P_2$ should obtain state
 $(\mathbb{I} \otimes \sigma_2 \otimes\cdots \otimes \sigma_n) \ket{\Psi}_{\sfP_1, \sfP_{1,2}',\cdots  \sfP_{1,n}'}$ in registers $\sfP_1,\sfP_{1,2}',\cdots, \sfP_{1,n}'$ in its $\ell_{1,2}^*$-th register in $\sfP_{2}^{N_{1,2}}$, namely, register $\sfP_{2, \ell_{1,2}^*}$.
 
    \item Recall that $P_2$ holds the regular teleportation measurement outcome $\sigma_2$. Now it applies $\mathbf{I} \otimes \sigma_2 \otimes \cdots \mathbf{I}$ on all registers in $\sfP_{2}^{N_{1,2}}$.

    \item  Now we generalize the above to the rest of the parties:  

    For $i \in \{2,\cdots n-1\}$
    \begin{enumerate}
    \item  Recall that each neighboring party $P_i$ and $P_{i+1}$ shares $nk$-bits of maximal entanglement in each register $\sfP_{i,R,\ell_{i,i+1}}: \sfP_{i+1, L,\ell_{i,i+1}}$ among the register emsembles $\sfP_{i,R}^{N_{i,i+1}} :\sfP_{i+1,L}^{N_{i,i+1}}$.
    We set $N_{i,i+1} = O(2^{N_{i-1,i}})$ \footnote{More specifically, $N_{i,i+1} = O(2^{8N_{i-1,i}+4} /\epsilon^2)$  where $\epsilon$ is an accuracy factor in the implementation of port based measurement.}. 
    
    $P_i$ performs the following:
    
    \item $P_i$ performs a port-based teleportation measurement for each of its register in $\sfP_{i,R}^{N_{i-1,i}}$: 
    on its $nk$-qubits in register  $\sfP_{i,L, \ell_{i-1,i}}$
    and its part of the shared entanglement
    in registers $\sfP_{i,R,2^{\ell_{i-1,i}}+1} \sfP_{i,R,2^{\ell_{i-1,i}}+2} \cdots \sfP_{i,R,2^{\ell_{i-1,i}+1}} : \sfP_{i+1,L, 2^{\ell_{i-1,i}}+1}, \sfP_{i+1,L, 2^{\ell_{i-1,i}}+1} \cdots \sfP_{i+1,L, 2^{\ell_{i-1,i}+1}}$.

    
  \item  Party $P_i$ obtains $N_{i-1,i}$ measurement outcomes $t_{i,i+1}^1, \cdots, t_{i,i+1}^{N_{i-1,i}}$. Each $t_{i,i+1}^j, j \in [N_{i-1,i}]$ is an index in $[1,2,\cdots, N_{i,i+1}]$. 
    Now, party $P_{i+1}$ should obtain state
 $(\mathbb{I} \otimes \mathbb{I} \otimes \cdots \otimes \sigma_{i+1} \otimes \cdots \otimes \sigma_n) \ket{\Psi}_{\sfP_1, \sfP_{1,2}',\cdots \sfP_{1,n}'}$ in one of its registers among $\sfP_{i+1,L}^{N_{i,i+1}}$.
It applies $\mathbb{I} \otimes \mathbb{I} \otimes \cdots \otimes \sigma_{i+1} \otimes \cdots \otimes \mathbb{I}$ on all registers in $P_{i+1,L}^{N_{i,i+1}}$.
 
 %registers $P_1,P_{1,2}',\cdots P_{1,n}'$ in %\its $\ell_{1,2}^*$-th register in $P_{2}^{N_{1,2}}$, namely, register $P_{2, \ell_{1,2}^*}$.

    \end{enumerate} 
    
\item At the end of the above sequential operations, party $P_n$ obtains the  state $(\mathbb{I} \otimes \mathbb{I} \otimes \cdots \otimes \sigma_n) \ket{\Phi}_{\sfP_1, \sfP_{1,2}',\cdots \sfP_{1,n}'}$ in one of its registers among $\sfP_{n,L}^{N_{n-1,n}}$. It applies $\mathbb{I} \otimes \mathbb{I} \otimes \cdots \otimes \sigma_n$ to all registers in $\sfP_{n,L}^{N_{n-1,n}}$; $P_n$ now holds the state $\ket{\Psi}_{\sfP_1, \sfP_{1,2}',\cdots \sfP_{1,n}'}$ in one of the registers. It applies the POVM measurement $\reconstruct_{\sfP_1 \sfP_2 \cdots \sfP_n}$ on all registers in $P_{n,L}^{N_{n-1,n}}$ and obtains $N_{n-1,n}$ number of measurement outcomes $\{\gamma_{j}\}_{j \in [N_{n-1,n}]}$.

 
   
    \end{enumerate}

\item Reconstruction stage:
For each party $P_i, i \in \{1,\cdots, n-1\}$, $P_i$ sends all measurement outcomes from its port teleportation measurement $\{t_{i,i+1}^k\}_{N_{i,i-1}}$ to both recoverers Bob and Charlie; for party $P_n$, it sends the measurement outcomes $\{\gamma_{j}\}_{j \in [N_{n-1,n}]}$ to Bob and Charlie. Bob and Charlie use these messages to recover the secret $m$.


\end{enumerate}
\pnote{I wouldn't use the term correctness here since this is an attack or you meant correctness of attack?}
\paragraph{Correctness of the Attack:}
The recoverers Bob and Charlie both obtain all measurement outcomes $\{t_{i,i+1}^k\}_{N_{i,i-1}}$ and $\{\gamma_{j}\}_{j \in [N_{n-1,n}]}$ since they are all classical.
By the correctness of the regular teleportation protocol and the port teleportation protocol, the secret $\gamma^*$ to be recovered should appear in one of the values $\{\gamma_{j}\}_{j \in [N_{n-1,n}]}$. 
Using the port teleportation outcomes, they can find out this correct register  and therefore the correct secret $\gamma^*$, which is the measurement outcome of $\{\reconstruct_{P_1, \cdots, P_n}^{\gamma}\}_{\gamma}$ applied on $\ket{\Psi}_{P_1, \cdots, P_n}$ performed by $P_n$.





\end{proof}



==> thresholdss.tex <==
\section{Threshold Unclonable Secret sharing}
\pnote{should we remove this?}

 Note: $t$ needs to be greater than $n/2$.

 \vipul{I changed $k$ to $t$}
 
 
 We give the following construction assuming an underlying unclonable encryption: 
\paragraph{Construction}
\begin{enumerate}
    \item Use a classical $t$-out-of-$n$ secret-sharing scheme to secret share $m$. (e.g. Shamir)
    
    \item Sample random $y_i, y_i' $ for all $i \in [n]$.
    
    \item Compute $\sk_i = H(y_i, y_i')$ using random oracle $H$.
    
    \item Use unclonable encryption $\enc(\sk_i, m_i) \to \ket{\ct_{m_i}}$. 
    
    \item Give share $(y_i, \ket{\ct_{m_i}})$ to party $P_i$. Additionally, give $y_i'$ to all parties $P_j$, for $j \neq i$.
    
\end{enumerate}

\vipul{In the above construction, the total share size is $n^2$. It's easy to reduce it to $n(n-t+1)$ (Just have $n-t+1$ parties encrypt their shares using uncloneable encryption, the other shares are stored by the respective parties as it is. This still guarantees that for any authorized set, at least 1 party has it's share under uncloneable encryption.) But can we do better?}

\vipul{Here is an idea for better share size: prepare a packed secret sharing of all $y_i'$ and give the shares to $n$. Reconstruction threshold = $t$ and packing parameter (i.e., number of secrets stored in a single polynomial) can be say $n/4$. This should yield O(n) total share size.}

\vipul{Can we get collusion resistance? Rather than giving $y_i'$ to all other parties, maybe we secret share it using $k$ out of $n$ secret sharing?}
